Sparse Full Configuration Interaction

We propose an efficient deterministic method to calculate the full configuration interaction (FCI) ground state energy. This method leverages the sparseness of the Lanczos basis vectors that span the Krylov subspace associated with the Hamiltonian to rapidly calculate the lowest eigenvalue of the effective Hamiltonian formed in this basis. By iteratively performing the spanning and diagonalization steps, this method is capable of rapidly reaching chemical accuracy for a variety of strongly correlated molecules, including stretched N$_2$ and C$_2$, in merely several tens of iterations. To accelerate our algorithm, we implement parallelized sparse matrix-sparse vector multiplication, which features a novel hashing method that establishes a one-to-one correspondence between the set of full configuration Slater determinants and a set of consecutive integers. A near-linear acceleration was observed.

==> old.tex <==
In this work, we use the simplest criterion to truncate vectors. We expect that beyond truncating with respect to coefficient magnitude, more sophisticated selection criteria can improve the convergence. 

Right now, we fix $N_d$ for all $\ket{w_i}$. Adaptively adjusting $N_d$ 

Also, various matrix-vector multiplication techniques are trasnferable to the context of SFCI, which can lead to further enhancement in performance, as well as the applicable system size. 



Previously, two indexing methods were proposed to my knowledge. The first one was to simply generate the FCI vector and build a hash table. Since this way requires the storage of the full FCI vector, it is not viable in our setting. The second is to divide a bit-string that represents an electronic configuration into two equally long sub-strings. Then, a hash table for the sub-string is constructed, and the index of the original string is computed from the indices of the two substrings. In comparison with the first approach, this approach significantly reduces the storage and turned out to be very helpful in the early days of computational physics when computer memory was tiny by today's standards. However, in our setting, this approach is still not efficient enough.  

The indexing method is somehow related to another issue in quantum chemistry. Despite its wide usage, the bit-string is known to be a ``sparse” representation of a determinant, in the sense that much of the encoding space is wasted. For example, though a 4 Byte integer type can encode up to $2^{32}$ different integers, it can only represent determinants with no more than 32 spin orbitals, regardless of the number of electrons. When the electron number is small, a huge fraction of the encoding space is in fact unused. 

Here, I present a compact indexing of determinants. It is compact in the sense that it is in fact a one-to-one and onto mapping between [det1, det2,…detN] and a set of consecutive integers [0,1,…, N-1], in which $N$ is the total number of determinants. 
 
It is helpful to think of indexing a determnant as determining how far it has traveled from an initial state. I define a bit-string as ``initialized” when all its 1s are on the left, such as 11…11000…000. Likewise, a “final” state is defined to be a string in which all 1s stay on the right, such as 0000…001111..11. \cite{introsort}

As long as we map the initial state to 0, we can calculate the index of any determinant by calculating the ``distance” it has traveled. The rule for traveling is defined recursively. One first starts from the leftmost (the 1st) "1" in the string, and check if the bit on its right is 0. If yes, a single move is accomplished; if not, look for the 2nd "1" and stop until a move is made. After each move, one should also “reset” all "1"s left to the "1" that has just been moved. For example,  the next bit-string of “011101” should be “110011”, since the 3rd "1"s is moved 1 bit rightward, and the 1st and 2nd "1"s should be reset to their initial positions. 

The following graph shows for a 5-orbital 3-electron system, how the initial configuration moves step-by-step to the final configuration. 

\begin{equation}
\begin{aligned}
& 11100 \rightarrow 11010 \rightarrow 10110 \rightarrow 01110 \rightarrow 11001  \\
		\rightarrow & 10101 \rightarrow 01101 \rightarrow 10011 \rightarrow 01011 \rightarrow 00111 
\end{aligned}
\end{equation}	

Given this rule, we may compute the distance that any configuration has traveled from the initial state. Suppose we have a configuration "101010", and we start with the 3rd "1" which lives in orbital 5. Regarding this bit, there must be at least $\binom{5-1}{3}$ configurations before it. The reason is that orbital 5 can be 1 only after all configurations with all 3 "1"s living in the fist 4 orbitals has been exhausted. Likewise, for the 2nd and the 1st "1", the values are $\binom{3-1}{2}$ and $\binom{1-1}{1}$ respectively. For the uniformity of expression, an n-choose-k with n smaller than k is allowed, and is defined to be 0, since, there is apparently no way to choose 2 elements out of only 1 element. Thus, the index of configuration "101010" is 

$$\binom{4}{3} + \binom{2}{2} + \binom{0}{1} = 5$$


As an example, indexing determinants with 6 orbitals and 3 electrons is shown below. 

$$111000 \rightarrow \binom{2}{3} + \binom{1}{2} +\binom{0}{1}  =0+0+0 = 0 $$

$$110100 \rightarrow \binom{3}{3} + \binom{1}{2} +\binom{0}{1}  = 1+0+0=1 $$

$$101100 \rightarrow \binom{3}{3} + \binom{2}{2} +\binom{0}{1}  = 1+1+0=2 $$

$$011100 \rightarrow \binom{3}{3} + \binom{2}{2} +\binom{1}{1}  = 1+1+1=3 $$

$$110010 \rightarrow \binom{4}{3} + \binom{1}{2} +\binom{0}{1}  = 4+0+0=4 $$

$$101010 \rightarrow \binom{4}{3} + \binom{2}{2} +\binom{0}{1}  = 4+1+0=5 $$

$$011010 \rightarrow \binom{4}{3} + \binom{2}{2} +\binom{1}{1}  = 4+1+1=6 $$

$$100110 \rightarrow \binom{4}{3} + \binom{3}{2} +\binom{0}{1}  = 4+3+0=7 $$

$$010110 \rightarrow \binom{4}{3} + \binom{3}{2} +\binom{1}{1}  = 4+3+1=8 $$

$$001110 \rightarrow \binom{4}{3} + \binom{3}{2} +\binom{2}{1}  = 4+3+2=9 $$

$$110001 \rightarrow \binom{5}{3} + \binom{1}{2} +\binom{0}{1}  = 10+0+0=10 $$

$$101001 \rightarrow \binom{5}{3} + \binom{2}{2} +\binom{0}{1}  = 10+1+0=11 $$

$$011001 \rightarrow \binom{5}{3} + \binom{1}{2} +\binom{1}{1}  = 10+1+1=12 $$

$$100101 \rightarrow \binom{5}{3} + \binom{3}{2} +\binom{0}{1}  = 10+3+0=13 $$

$$010101 \rightarrow \binom{5}{3} + \binom{3}{2} +\binom{1}{1}  = 10+3+1=14 $$

$$001101 \rightarrow \binom{5}{3} + \binom{3}{2} +\binom{2}{1}  = 10+3+2=15 $$

$$100011 \rightarrow \binom{5}{3} + \binom{4}{2} +\binom{0}{1}  = 10+6+0=16 $$

$$010011 \rightarrow \binom{5}{3} + \binom{4}{2} +\binom{1}{1}  = 10+6+1=17 $$

$$001011 \rightarrow \binom{5}{3} + \binom{4}{2} +\binom{2}{1}  = 10+6+2=18 $$

$$000111 \rightarrow \binom{5}{3} + \binom{4}{2} +\binom{3}{1}  = 10+6+3=19 $$

Note that all n-choose-k values can be prepared at the initial stage. When calculating index, these values are fetched when needed. Such a value table is of trivial size. For a system with M electrons and N orbitals, the space required for the table is 2*N*M. 

The above indexing process shows how to efficiently \textit{encode} a bit-string in an integer. Similarly, one can efficiently \textit{decode} an integer to obtain the corresponding bit-string. Suppose we ask what is the corresponding determinant of integer 15. One can refer to the nchoosek table in Figure 2. One first checks the last column and finds that 15 is greater than 10 and smaller than 20. This indicates that the 3rd electron is in orbital 6. Next, ones find that the difference of 15 and 10, which is 5, is greater than 3 and smaller than 6, and works out that the 2nd electron is in orbital 4. This process continues until electrons are exhausted. 


\begin{figure}
	\centering
	\includegraphics[width=0.80\linewidth]{table.png}
	\caption{A n-choose-k table}
\end{figure}




We will consider \textit{ab initio} Hamiltonians that contain up to double excitations. In the language of second quantization, the Hamiltonian can be written as: 

$$\hat{H} = H_0 + \sum_{m,n}C_{mn}\hat{a}_m^\dagger\hat{a}_n+\sum_{m,n,p,q}C_{mnpq}\hat{a}_m^\dagger\hat{a}_n\hat{a}_p^\dagger\hat{a}_q$$

Determinents are represented as bit-strings.  

Suppose one has a single determinant $\ket{\chi_1 \chi_2 ... \chi_N}$, where $N$ is \BR{Define N}. Applying $\hat{H}$ on this determinant yields a set of determinants that consists of the original determinant, single excitations, and double excitations. That is, 

$$\hat{H} \ket{\chi_1 \chi_2 ... \chi_N} = H_0\ket{\chi_1 \chi_2 ... \chi_N} + \sum_i \alpha_i \ket{single \ excitation\ i} + \sum_j \beta_j \ket{double\ excitation\ j}$$

Naturally, the resultant set of determinants can be written as a vector of determinants. 

$$\hat{H} \ket{\chi_1 \chi_2 ... \chi_N} = \sum_k C_k \ket{k}$$

In comparison to a FCI vector, which is typically dense, the resultant vector of this operation is a sparse one. Therefore, a sparse matrix sparse vector formalism should be adopted when calculating scenarios shown above. 

The central idea of SFCI is to use an iterative method (Davidson, Lanczos, etc.)to find the ground state while keeping all of the vectors sparse. In other words, any vector is allowed to contain no more than $N_d$ determinants (and their corresponding coefficients). Vectors having more than this number of determinants will be truncated, so that only $N_d$ of the most important determinants remain. For example, if the vector $\ket{\psi_0}$ has $N_d$ determinants, 

$$\ket{\psi_0} = \sum_{i=1}^{N_d} C_i\ket{i}$$
and $\ket{\psi_1}$ is the resultant vector after applying $\hat{H}$ to $\ket{\psi_0}$


\begin{equation}
\begin{aligned}
\ket{\psi_1} &= \hat{H} \ket{\psi_0} \\
			& = \sum_{j=1}^{M} D_j \ket{j} 
\end{aligned}
\end{equation}	
with $M$ greater than $N_d$, then, only the $N_d$ most important $\ket{j}$ measured by $|D_j|$ will be kept in memory. Likewise, the same criterion for truncation must also be applied in operations such as vector addition.

We find that with a reasonable choice of $\epsilon$, truncating the result vector of SpMSpV with respect to the determinant coefficients has nearly no impact to the result. The overall execution time, however, can be  shortened significantly, due to the decreased workload of sorting. For C2 cc-pVDZ calculation with ($\epsilon = 5 \times 10^{-6}$ Ha) and without SpMSpV result vector truncation, the convergence time are 8 minutes and 12 minutes respectively. The converged energies are almost identical. 

